Quality Competition Among Internet Service Providers

Internet service providers (ISPs) have a variety of quality attributes that determine their attractiveness for data transmission, ranging from quality-of-service metrics such as jitter to security properties such as the presence of DDoS defense systems. ISPs should optimize these attributes in line with their profit objective, i.e., maximize revenue from attracted traffic while minimizing attribute-related cost, all in the context of alternative offers by competing ISPs. However, this attribute optimization is difficult not least because many aspects of ISP competition are barely understood on a systematic level, e.g., the multi-dimensional and cost-driving nature of path quality, and the distributed decision making of ISPs on the same path. In this paper, we improve this understanding by analyzing how ISP competition affects path quality and ISP profits. To that end, we develop a game-theoretic model in which ISPs (i) affect path quality via multiple attributes that entail costs, (ii) are on paths together with other selfish ISPs, and (iii) are in competition with alternative paths when attracting traffic. The model enables an extensive theoretical analysis, surprisingly showing that competition can have both positive and negative effects on path quality and ISP profits, depending on the network topology and the cost structure of ISPs. However, a large-scale simulation, which draws on real-world data to instantiate the model, shows that the positive effects will likely prevail in practice: If the number of selectable paths towards any destination increases from 1 to 5, the prevalence of quality attributes increases by at least 50%, while 75% of ISPs improve their profit.

==> archive/overcomplicated-proof.tex <==
 In a first attempt, we try to find the unrestricted maximizing attributes~$\mathbf{\hat{A}}^{**}$ by means of the first derivative,
    which leads to the following system of equations:
    \begin{align}
        \forall n \in r, k \in [K].\quad &\frac{\partial}{\partial a_{nk}} \sum_{n \in r} \pi_n(\mathbf{\hat{A}}^{**}) = 0
        \iff& v_r(\mathbf{\hat{A}}^{**}) =  \sqrt{\frac{\alpha_{nk}}{\gamma_{nk}}} \sqrt{d\sum_{n\in r} (\rho_n - \phi_{n0})} - 1 \label{eq:theo:sapp-constant:single-path:optimum:2}
    \end{align}
    We make two observations regarding that system of equations. 
    
    First, the equation system can only be solved if all attributes~$(n,k)$ are associated
    with the identical ratio~$\alpha_{nk}/\gamma_{nk}$. In that case, all~$\mathbf{\hat{A}}^{**}$ 
    such that~$v_r(\mathbf{\hat{A}}^{**})$ amounts to the quantity above solve the system.
    In contrast, for non-identical ratios, the aggregate-profit function is unbounded,
    and only the equations for a single ratio~$\alpha_{nk}/\gamma_{nk}$ can hold at any time
    (Note that multiple attributes may be associated with the same ratio).
    
    Second, considering the restricted domain~$\mathbb{R}_{\geq 0}$, the equation specific to a ratio~$\alpha_{nk}/\gamma_{nk}$ 
    cannot possibly hold under the following condition:
    \begin{equation}
        \alpha_{r0} > \sqrt{\frac{\alpha_{nk}}{\gamma_{nk}}} \sqrt{d\sum_{n\in r} (\rho_n - \phi_{n0})} - 1
        \label{eq:theo:sapp-constant:single-path:optimum:4}
    \end{equation}
    If that condition holds for all~$n\in r$ and $k \in [K]$, then~$\mathbf{A}^{**} = \boldsymbol{0}$
    maximizes the aggregate profit function. To confirm this statement, consider the socially optimal~$\hat{a}_{nk}^{**}$
    given all other attribute values~$\mathbf{A}_{-nk}$, derived from~\cref{eq:theo:sapp-constant:single-path:optimum:2}:
    \begin{equation}
        \hat{a}_{nk}^{**}(\mathbf{A}_{-nk}) = \frac{\sqrt{\frac{\alpha_{nk}}{\gamma_{nk}}} \sqrt{d\sum_{n\in r} (\rho_n - \phi_{n0})} - (1 + \sum_{(n',k') \in r\times [K]. (n',k') \neq (n,k)} \alpha_{n'k'} a_{n'k'} +\alpha_{r0})}{\alpha_{nk}}
    \end{equation}
    For~$\mathbf{A}_{-nk} = \boldsymbol{0}$ and the condition in~\cref{eq:theo:sapp-constant:single-path:optimum:4},
    it holds for all~$n \in r$ and~$k \in [K]$ that $\hat{a}_{nk}^{**}(\boldsymbol{0}) < 0$.
    Since~$a_{nk}^{**}(\mathbf{A}_{-nk}) = \max(0, \hat{a}_{nk}^{**}(\mathbf{A}_{-nk}))$
    thanks to the concavity of the aggregate-profit function,
    consistently zero-valued attributes thus optimize the aggregate-profit function
    if no equation in the system of~\cref{eq:theo:sapp-constant:single-path:optimum:2} is solvable.
    
    Now we consider the case where at least one equation in the equation system of~\cref{eq:theo:sapp-constant:single-path:optimum:2}
    is solvable on the restricted domain. It is easy to see that if some equations in the systems can be solved,
    then the profit-optimizing~$\mathbf{A}^{**}$ in fact solves one equation, specific to a ratio~$\alpha_{nk}/\gamma_{nk}$:
    For the sake of contradiction, let~$\mathbf{A}^{**}$ be profit-maximizing attribute values that do not solve any
    of the solvable equations, i.e.,
    \begin{equation}
        \forall n \in r, k \in [K] \text{ with } \alpha_{r0} \leq  \sqrt{\frac{\alpha_{nk}}{\gamma_{nk}}}\sqrt{d\sum_{n\in r} (\rho_n - \phi_{n0})} - 1. 
        \quad \frac{\partial}{\partial a_{nk}} \sum_{n \in r} \pi_n(\mathbf{A}^{**}) \neq 0.
    \end{equation}
    In that case, any~$a_{nk}$ corresponding to a solvable equation could be adjusted to satisfy the respective equation,
    leading to a profit improvement because the aggregate-profit function is concave in any attribute value.
    Thereby, we have a contradiction with the profit-maximizing character of~$\mathbf{A}^{**}$.
    
    If solvable equations exist, the profit-maximizing attribute values~$\mathbf{A}^{**}$ thus solve
    one of those equations. Let~$(n^{**}, k^{**}) \in r\times [K]$ be the attribute that is associated with the ratio
    for which~$\mathbf{A}^{**}$ solves the corresponding equation, i.e.,
    \begin{equation}
        v_r(\mathbf{A}^{**}) =  \sqrt{\frac{\alpha_{n^{**}k^{**}}}{\gamma_{n^{**}k^{**}}}} \sqrt{d\sum_{n\in r} (\rho_n - \phi_{n0})} - 1.
        \label{eq:theo:sapp-constant:single-path:optimum:4}
    \end{equation}
    Then, we can reformulate our optimization problem as follows:
    \begin{equation}
        \begin{aligned}
        \mathbf{A}^{**} = {\arg\max}_{\mathbf{A} \in \mathbb{R}_{\geq} 0} \sum_{n\in r} \pi_n(\mathbf{A}) =&\ {\arg\min}_{\mathbf{A} \in \mathbb{R}_{\geq} 0} \sum_{n\in r}\sum_{k \in [K]}\gamma_{nk} a_{nk} 
        \\
        &\ \text{ subject to }  v_r(\mathbf{A}) = \sqrt{\frac{\alpha_{n^{**}k^{**}}}{\gamma_{n^{**}k^{**}}}} \sqrt{d\sum_{n\in r} (\rho_n - \phi_{n0})} - 1.
    \end{aligned}
    \label{eq:theo:sapp-constant:single-path:optimum:5}
    \end{equation}
    
    The constraint in the reformulated optimization problem means that for all $n' \in [r]$ and $k' \in [K]$:
    \begin{align}
       a_{n'k'} =&\ \frac{1}{\alpha_{n'k'}}\left( \sqrt{\frac{\alpha_{n^{**}k^{**}}}{\gamma_{n^{**}k^{**}}}} \sqrt{d\sum_{n\in r} (\rho_n - \phi_{n0})} - (1 + \sum_{\substack{(n,k) \in r\times[K].\\(n,k) \neq (n',k')}} \alpha_{nk} a_{nk} + \alpha_0)\right)\\
       =:&\ \frac{1}{\alpha_{n'k'}}\left(T_{22} - \sum_{\substack{(n,k) \in r\times[K].\\(n,k) \neq (n',k')}} \alpha_{nk} a_{nk}\right)
    \end{align}
    
    This representation of the constraint allows the following interesting transformation,
    where~$(n',k')$ is an arbitrary attribute:
    \begin{align}
        \sum_{n\in r}\sum_{k \in [K]}\gamma_{nk} a_{nk} =&\ \sum_{\substack{(n,k) \in r\times[K].\\(n,k) \neq (n',k')}} \gamma_{nk} a_{nk} + \frac{\gamma_{n'k'}}{\alpha_{n'k'}} \left(T_{22} - \sum_{\substack{(n,k) \in r\times[K].\\(n,k) \neq (n',k')}} \alpha_{nk} a_{nk} \right)\\
        =&\ \sum_{\substack{(n,k) \in r\times[K].\\(n,k) \neq (n',k')}} \frac{\gamma_{nk}\alpha_{n'k'} - \gamma_{n'k'}\alpha_{nk}}{\alpha_{n'k'}} a_{nk} + \frac{\gamma_{n'k'}}{\alpha_{n'k'}} T_{22}
        \label{eq:theo:sapp-constant:single-path:optimum:6}
    \end{align}
    
    Now, we choose the attribute~$(n',k')$ as
    an attribute that is associated with
    the maximal ratio~$\alpha_{n'k'}/\gamma_{n'k'}$:
    \begin{equation}
        (n', k') = {\arg\max}_{(n,k) \in r\times[K]}
        \frac{\alpha_{nk}}{\gamma_{nk}}
    \end{equation}
    As a result, it holds that the coefficients
    of all~$a_{nk}$, $(n,k) \neq (n',k')$, in~\cref{eq:theo:sapp-constant:single-path:optimum:6}
    are not negative:
    \begin{equation}
        \forall (n,k) \in r\times[K], (n,k) \neq (n',k').\quad
        \frac{\alpha_{n'k'}}{\gamma_{n'k'}} \geq \frac{\alpha_{nk}}{\gamma_{nk}} \iff \gamma_{nk}\alpha_{n'k'} - \gamma_{n'k'}\alpha_{nk} \geq 0 
    \end{equation}
    Hence,~\cref{eq:theo:sapp-constant:single-path:optimum:6}
    is minimized by setting~$a_{nk} = 0$ for all 
    attributes~$(n,k) \neq (n',k')$ 
    with~$\alpha_{nk}/\gamma_{nk} < \alpha_{n'k'}/\gamma_{n'k'}$.
    All attributes~$(n,k) \in r\times[K]$ with the maximal ratio~$\alpha_{nk}/\gamma_{nk} = \alpha_{n'k'}/\gamma_{n'k'}$
    form the set~$K^{**}$, and have values~$a_{nk} \geq 0$ satisfying the constraint in~\cref{eq:theo:sapp-constant:single-path:optimum:5}.
    
    In summary, the attribute values~$\mathbf{A}^{**}$ need to have the following properties in order to maximize the aggregate profit:
    \begin{align}
        &\forall (n,k) \in K^{**}.\quad a_{nk}^{**} \geq 0 \hspace{40pt} \forall (n,k) \notin K^{**}.\quad a_{nk}^{**} = 0 \label{eq:theo:sapp-constant:single-path:optimum:9}\\
        &v_r(\mathbf{A}^{**}) =  \sqrt{\frac{\alpha_{n^{**}k^{**}}}{\gamma_{n^{**}k^{**}}}} \sqrt{d\sum_{n\in r} (\rho_n - \phi_{n0})} - 1
        \label{eq:theo:sapp-constant:single-path:optimum:7}
    \end{align}
    To further qualify this optimum, we need to identify the ratio~$\alpha_{n^{**}k^{**}}/\gamma_{n^{**}k^{**}}$
    for which the equation in the system from~\cref{eq:theo:sapp-constant:single-path:optimum:2} is solved.
    
    To identify this ratio, we observe the profit-maximizing attribute values~$\mathbf{A}^{**}$ 
    lie at the boundary with respect to all~$(n,k) \notin K^{**}$, suggesting:
    \begin{equation}
        \forall (n,k) \in K^{**}.\quad \frac{\partial}{\partial a_{nk}} \sum_{n\in r} \pi_n(\mathbf{A}^{**})
        = 0 \hspace{40pt} \forall (n,k) \notin K^{**}.\quad \frac{\partial}{\partial a_{nk}} \sum_{n\in r} \pi_n(\mathbf{A}^{**})
        < 0 
    \end{equation}
    The first of these conditions can be transformed to the same form as in~\cref{eq:theo:sapp-constant:single-path:optimum:2}:
    \begin{align}
        \forall (n,k) \in K^{**}.\quad&\ \frac{\partial}{\partial a_{nk}} \sum_{n \in r} \pi_n(\mathbf{A}^{**}) =  0 
        \iff v_r(\mathbf{A}^{**}) = \sqrt{\frac{\alpha_{nk}}{\gamma_{nk}}} \sqrt{d\sum_{n\in r} (\rho_n - \phi_{n0})} - 1
        \label{eq:theo:sapp-constant:single-path:optimum:8}
    \end{align}
    
    Together, \cref{eq:theo:sapp-constant:single-path:optimum:7} and \cref{eq:theo:sapp-constant:single-path:optimum:8}
    suggest that~$\mathbf{A}^{**}$ solves the equation in the system from~\cref{eq:theo:sapp-constant:single-path:optimum:2} 
    associated with the maximum ratio~$\alpha_{nk}/\gamma_{nk}$:
    \begin{equation}
        \forall (n,k) \in K^{**}. \quad
        \frac{\alpha_{n^{**}k^{**}}}{\gamma_{n^{**}k^{**}}} = \frac{\alpha_{nk}}{\gamma_{nk}} = \max_{(n',k') \in r\times[K]} \frac{\alpha_{n'k'}}{\gamma_{n'k'}}
    \end{equation}
    
    We have thus identified the conditions on~$\mathbf{A}^{**}$ necessary for optimal aggregate profit.
    To be a Nash bargaining solution, $\mathbf{A}^{**}$ additionally needs to be maximally fair, i.e.,
    the profit distribution across nodes must be as equal as possible.
    This maximum fairness is achieved by optimizing the Nash bargaining product
    subject to the constraints in~\cref{eq:theo:sapp-constant:single-path:optimum:7,eq:theo:sapp-constant:single-path:optimum:9}, i.e.:
    \begin{equation}
        \mathbf{A}^{**} = {\arg\max}_{\mathbf{A} \in \mathbb{R}_{\geq 0}} \Pi_{n \in r} \pi_{n}(\mathbf{A}) \text { subject to \cref{eq:theo:sapp-constant:single-path:optimum:7,eq:theo:sapp-constant:single-path:optimum:9}.} 
    \end{equation}
    
    Thereby, the theorem is proven.

==> makefile <==
FILES = paper
# FILES = $(patsubst %.tex,%,$(wildcard *.tex))
FILES_PDF = $(addsuffix .pdf,$(FILES))
FILES_FINAL_PDF = $(addsuffix -final.pdf,$(FILES))
FILES_DIFF_PDF = $(addsuffix -diff.pdf,$(FILES))

.PHONY: $(FILES_PDF) $(FILES_FINAL_PDF) $(FILES_DIFF_PDF) all clean final diff.pdf

all: $(FILES_PDF) $(FILES_FINAL_PDF)

final: $(FILES_FINAL_PDF)

$(FILES_PDF): %.pdf: %.tex
	latexmk -pdf -jobname=$(basename $@) -bibtex --synctex=1 -shell-escape $<

$(FILES_FINAL_PDF): %-final.pdf: %.tex
	latexmk -pdf -jobname=$(basename $@) -bibtex --synctex=1 -shell-escape -pdflatex='pdflatex %O -interaction=nonstopmode -synctex=1 "\newcommand{\final}{}\input{%S}"' $<


P = paper

# default : $P.pdf

# $P.dvi	: $(wildcard *.tex *.bib figures/*.eps)
# 	latex  $P < /dev/null || $(RM) $@
# 	bibtex $P < /dev/null || $(RM) $@
# 	latex  $P < /dev/null || $(RM) $@
# 	latex  $P < /dev/null || $(RM) $@

# $P.pdf  : $(wildcard *.tex *.bib figures/*)
# 	pdflatex --shell-escape $P
# 	bibtex $P
# 	pdflatex --shell-escape $P
# 	pdflatex --shell-escape $P

# $P.ps	: $P.dvi
# 	dvips -tletter -Ppdf $P.dvi -o $P.ps

# $P.ps.gz: $P.ps
# 	$(RM) $P.ps.gz
# 	gzip -9 < $P.ps > $P.ps.gz

# print:	$P.ps

# dist:	$P.ps.gz

clean:
	$(RM) *.log *.aux *.bbl *.blg *.out *.dvi *.ps *.ps.gz *.fdb_latexmk *.synctex.gz *.fls texput.log


==> sections/a01-arbitrary-2path-sapp-derivation.tex <==
\section{Equilibrium Derivation for Arbitrary 2-Path Parallel-Path Network}
\label{app:arbitrary-2path-sapp}

Given a general parallel-path network with two paths~$r_1$ and~$r_2$,
where each path~$r_i$ contains exactly one node~$n_i$, the equilibrium
attribute~$a_1^+$ (of node~$n_1$) can be found with the following equation:
\begin{equation}
    a_1^{+} = a_1^{\ast}\big(a_2^{\ast}(a_1^+)\big)
\end{equation} where~$a_1^{\ast}$ yields the optimal
choice for attribute~$a_1$ given attribute~$a_{2}$,
and vice versa for~$a_2^{\ast}$
(cf.~\cref{thm:sapp:a_opt}). Under the initial assumption 
that~$a_1^+,\ a_2^+ \geq 0$,
this equation can be transformed into the following 
labyrinthine equation that is quartic in~$a_1^+$
and does not permit a straightforward analytic solution:
\begin{equation}
    T_4 {a_1^+}^4 + T_3 {a_1^+}^3 + T_2 {a_1^+}^2 + T_1 a_1^+ + T_0 = 0
\end{equation} where
\begin{align}
    T_4 = &\alpha_{1}^{4}\left(\phi_{11}\left(2\phi_{21}\left(2\phi_{11}L_{1}+L_{2}\right)-\phi_{11}\right)-\phi_{21}^{2}L_{2}^{2}\right)\\
    T_3 = &2\alpha_{1}^{3}\left(\phi_{11}\left(2L_{1}\left(\phi_{11}L_{3}+\phi_{21}L_{5}\right)+L_{2}L_{3}-L_{5}\right)+\phi_{21}\left(L_{2}L_{5}-L_{2}^{2}L_{3}\right)\right)\\
    T_2 = &\alpha_{1}^{2}\big(L_{1}\left(4\phi_{11}^{2}L_{4}+4\phi_{11}L_{3}L_{5}+\phi_{21}L_{5}^{2}\right)-L_{2}^{2}\left(2\phi_{21}L_{4}+L_{3}^{2}\right)\\
    &+2L_{2}\left(\phi_{11}L_{4}+L_{5}L_{3}+\phi_{21}\alpha_{1}L_{6}\right)-2\phi_{11}\alpha_{1}L_{6}-L_{5}^{2}\big)\\
    T_1 = &\alpha_{1}\left(L_{1}\left(4\phi_{11}L_{4}L_{5}+L_{5}^{2}L_{3}\right)-2L_{2}^{2}L_{3}L_{4}+2L_{2}\left(L_{5}L_{4}+\alpha_{11}L_{3}L_{6}\right)-2\alpha_{1}L_{5}L_{6}\right)\\
    T_0 = &L_{1}L_{4}L_{5}^{2}-L_{2}^{2}L_{4}^{2}+2\alpha_{11}L_{2}L_{4}L_{6}-\alpha_{1}^{2}L_{6}^{2}
\end{align} which in turn rely on the following shorthands:
\begin{align}
    L_1 = & \frac{d}{d\phi_{21}+\gamma_{21}}\\
    L_2 = & \frac{\gamma_{11}}{d\phi_{21}+\gamma_{21}}\\
    L_3 = & \phi_{21}\left(2+2\alpha_{10}+\alpha_{20}\right)-\alpha_{2}\left(\phi_{20}-r_{2}\right)\\
    L_4 = & \left(1+\alpha_{10}\right)\left(\phi_{21}\left(1+\alpha_{10}+\alpha_{20}\right)+\alpha_{2}\left(r_{2}-\phi_{20}\right)\right)\\
    L_5 = & \phi_{11}\alpha_{10}-\alpha_{11}\left(r_{1}-\phi_{10}\right)\\
    L_6 = & -\alpha_{10}\left(r_{1}-\phi_{10}\right)
\end{align}

Moreover, if the equation above yields negative values for~$a_1^+$ or~$a_2^+$,
an equilibrium may be found by setting~$a_1^+ = a_1^{\ast}(0)$
and verifying that~$a_2^{\ast}(a_1^{\ast}(0)) \leq 0$ (and vice versa as well).

==> sections/proofs/homogeneous--competition-braess.tex <==
\begin{proof}
    We begin the proof by characterizing the equilibrium for the extended network~$\mathcal{N}_4$. 
    Despite not being a homogeneous parallel-path network as usual in this section, the equilibrium
    attribute~$a^+$ for network~$\mathcal{N}_4$ can also be identified in a straightforward manner
    thanks to the symmetries in the underlying equation system.
    Concretely, the profit function~$\pi_n$ of each ISP~$n$
    is of the previously encountered form:
    \begin{equation}
        \pi_n(\mathbf{A}) = d_n(\mathbf{A}) (\rho - \phi_1 a_n - \phi_0) - \gamma_1 a_n - \gamma_0
    \end{equation}
    where the demand~$d_1$ carried by ISP~$n_1$ is (symmetrically for ISP~$n_2$):
    \begin{equation}
        d_1(\mathbf{A}) = \frac{v_{r_1}(\mathbf{A}) + v_{r_3}(\mathbf{A})}{1 + v_{r_1}(\mathbf{A})+ v_{r_2}(\mathbf{A}) + v_{r_3}(\mathbf{A})}
        = \frac{\alpha_1a_1 + \alpha_0 + \beta_1(a_1+a_2) + \beta_0}{1 + \alpha_1(a_1+a_2) + 2\alpha_0 + \beta_1(a_1+a_2) + \beta_0}
    \end{equation}
    
    Hence, the equilibrium attributes~$\mathbf{\hat{A}}^+$ satisfy the following equation 
    for ISP~$n_1$ and a symmetric equation for ISP~$n_2$:
    \begin{equation}
        \frac{(\alpha_1+\beta_1)(1+v_{r_2}(\mathbf{\hat{A}}^+))}{\left(1+\sum_{r\in R} v_r(\mathbf{\hat{A}}^+)\right)^2} (\rho - \phi_1 \hat{a}^+_1 - \phi_0) - \phi_1 d_1(\mathbf{\hat{A}^+}) - \gamma_1 = 0
    \end{equation}
    As a result, the unrestricted equilibrium attribute~$\hat{a}^+$ satisfies
    the following equation:
    \begin{align}
        \hat{a}^+ &= &\hat{a}^{\ast}(\hat{a}^+)& \hfill \label{eq:thm:braess:aopt}\\
        &= &\frac{1}{\alpha_{1}+\beta_{1}} \Big(&\sqrt{\frac{d\left(1+\left(\alpha_{1}\hat{a}^++\alpha_{0}\right)\right)}{d\phi_{1}+\gamma_{1}}\left(\phi_{1}\left(1+\left(\alpha_{1}+\beta_{1}\right)\hat{a}^++2\alpha_{0}+\beta_{0}\right)+\left(\alpha_{1}+\beta_{1}\right)\left(\rho-\phi_{0}\right)\right)} \hfill \nonumber\\
        && &-\left(1+\left(\alpha_{1}+\beta_{1}\right)\hat{a}^++2\alpha_{0}+\beta_{0}\right) \Big) \nonumber
    \end{align}
    
    Equivalent to~\cref{thm:sapp:a_opt} and~\cref{thm:theo:sapp-homogeneous:equilibrium}, the
    shared equilibrium attribute~$a^+$ can be derived as
    \begin{equation}
        a^+ = \begin{cases}
            0 & \text{if } \hat{a}^+ \text{ is undefined or } \hat{a}^+ < 0\\
            \hat{a}^+ & \text{otherwise,}
        \end{cases}
    \end{equation}
    where
    the unrestricted equilibrium attribute~$\hat{a}^+$ is
    \begin{align}
        \hat{a}^+ =\ &\frac{\sqrt{T_{11}^2 -4T_{10}T_{12}} - T_{11}}{2T_{10}}, \label{eq:thm:braess:eq}\\
        T_{10} =\ &4\left(\alpha_{1}+\beta_1\right)^{2}-\frac{d\phi_{1}}{d\phi_{1}+\gamma_1}\alpha_{1}\left(\alpha_{1}+\beta_1\right),\label{eq:theo:sapp-homogeneous:braess:equilibrium_1}\\
        T_{11} =\ &4\left(\alpha_{1}+\beta_1\right)\left(1+2\alpha_{0}+\beta_0\right)-\frac{d}{d\phi_{1}+\gamma_1} \cdot \\
        &\ \left(\alpha_{1}\phi_{1}\left(1+2\alpha_{0}+\beta_0\right)+\left(\alpha_{1}+\beta_1\right)\left(\phi_{1}\left(1+\alpha_{0}\right)+\alpha_{1}\left(\rho-\phi_{0}\right)\right)\right), \text{ and}\nonumber\\
        T_{12} =\ &\left(1+2\alpha_{0}+\beta_0\right)^{2}-\frac{d}{d\phi_{1}+\gamma_1}\left(1+\alpha_{0}\right)\left(\phi_{1}\left(1+2\alpha_{0}+\beta_0\right)+\left(\alpha_{1}+\beta_1\right)\left(\rho-\phi_{0}\right)\right). \label{eq:theo:sapp-homogeneous:braess:equlibrium_3}
    \end{align}

    Crucially for the proof, the unrestricted equilibrium attribute~$\hat{a}^+$
    is undefined if the discriminant in~\cref{eq:thm:braess:eq} is negative:
    \begin{align}
        T_{11}^2 -4T_{10}T_{12} < 0 \iff T_{13}(\beta_1) \beta_0^2 + \mathcal{O}(\beta_0) < 0 \text{ where}\\
         T_{13}(\beta_1) = \frac{d\phi_{1} \alpha_{1}}{d\phi_{1}+\gamma_{1}}\left(\frac{d\phi_{1}}{d\phi_{1}+\gamma_{1}} \alpha_{1}-4\left(\alpha_{1}+\beta_{1}\right)\right) < 0 \quad \forall \beta_1 > 0
    \end{align}
    The consistent negativity of~$T_{13}$ for all valid~$\beta_1 > 0$ implies that the discriminant of the
    unrestricted equilibrium term is negative for all~$\beta_0$ above some~$\beta_0^-(\beta_1)$.
    Hence, the unrestricted equilibrium attribute~$a^+$ is undefined if~$\beta_0 > \beta_0^-(\beta_1)$.

    It remains to show that~$a^+ = 0$ is actually the equilibrium in the case where the unrestricted equilibrium~$\hat{a}^+$ is undefined, 
    i.e., if $\beta_0 > \beta_0^{-}(\beta_1)$.
    If that proposition holds, then the equilibrium attribute~$a^+(\mathcal{N}_4)$ in the extended network 
    can always be reduced to 0 by choosing~$\beta_0$ high enough (i.e., larger than~$\beta_0^-(\beta_1)$), whereas
    the equilibrium attribute~$a^+(\mathcal{N}_3)$ for the basic network is never lower than $0$ because
    of the domain restriction. Hence, if~$a^+(\mathcal{N}_4) = 0$ can always be achieved, then
    $a^+(\mathcal{N}_4) \leq a^+(\mathcal{N}_3)$ can always be achieved.

    To show that~$a^+ = 0$ is an equilibrium if the unrestricted equilibrium~$\hat{a}^+$ is undefined,
    note that the undefinedness of~$\hat{a}^+$ suggests that~\cref{eq:thm:braess:aopt} has no solution.
    Hence, since the best-response function~$\hat{a}^*$ is continuous, it must hold that either (i)~$a > \hat{a}^*(a)$ or 
    (ii)~$a < \hat{a}^{*}(a)$ for all~$a \in \mathbb{R}$.
    We can exclude case~(ii), as~$a < \hat{a}^{*}(a)$ must be false in the limit for~$a \rightarrow \infty$:
    \begin{equation}
        \lim_{a \rightarrow \infty} \hat{a}^{\ast}(a) = \lim_{a \rightarrow \infty} \frac{1}{\alpha_1 + \beta_1} \left( \sqrt{\frac{d\phi_1}{d\phi_1 + \gamma_1} \alpha_1 (\alpha_1 + \beta_1) a^2 + \mathcal{O}(a) } - \left((\alpha_1+\beta_1)a + \mathcal{O}(a)\right)\right)
        = -\infty
    \end{equation}

    Then, given that~$\hat{a}^{*}(a) < a\ \forall a \in \mathbb{R}$, it also holds that~$\hat{a}^{*}(0) < 0$, i.e.,
    the best-response attribute for ISP~$n_1$ given attribute~$a_{n_2} = 0$ of ISP~$n_2$ is below 0, and vice versa.
    Since the profit function~$\pi_n$ is consistently concave, it thus holds that~$a_{n_1} = 0$ is the best-response attribute
    to~$a_{n_2} = 0$ on the restricted domain~$\mathbb{R}_{\geq 0}$. Hence,~$a^+ = 0$ is an equilibrium
    if~$\beta_0 > \beta_0^{-}(\beta_1)$, and the theorem is proven.
\end{proof}

==> sections/sigmetrics-reply.tex <==
\section{Reply to SIGMETRICS Reviews}
\label{sec:app:sigmetrics-reviews}

We thank all reviewers for their detailed and insightful reviews,
which significantly helped improve the paper.
In addition to substantial rewriting of the paper body and the proofs, 
we have addressed the suggestions by the reviewers as follows:

\paragraph{Applicability to today's operational networks}
In the former version of our paper, we applied our new competition
model specifically to emerging path-aware network (PAN) architectures,
which allow inter-domain path selection by 
end-hosts~\cite{anderson2013nebula,barrera2017scion,bhattacharjee2006postmodern,filsfils2018segment,godfrey2009pathlet,raghavan2008secure,yang2007nira}.
While some PAN deployments exist~\cite{six2022ssfn,ladines2023hin},
these deployments are arguably still limited.
However, our model is general enough to accommodate
path selection by ISPs (instead of end-hosts) and
thus for an application to today's Internet, which
is based on the Border Gateway Protocol (BGP).
Such an application to a BGP-based Internet is
provided by the paper version at hand, which therefore
has straightforward practical relevance.

To further increase the usefulness of our insights
for real-world ISPs, we have additionally formulated
concrete business-strategy recommendations for ISPs
in the conclusion~(\cref{sec:conclusion}).
These recommendations help ISPs navigate the
competition under attribute-oriented path selection,
namely by identifying attractive quality attributes for investment
and by informing the interaction with other ISPs.

\paragraph{Clarification of model}
We have clarified our model and its assumptions
in multiple respects (\cref{sec:model}). 
First, we have restructured
the notation for demand associated with ISPs,
paths, and ISP pairs, respectively.
Second, we have demonstrated how an ISP's forwarding
price can affect ISP revenue and demand in our model, 
namely by its inclusion as an
`undesirable' quality attribute.
Third, we have demonstrated by
simulation that the model predictions
are not highly sensitive to
the assumption of affine functions
for valuation and cost, especially
regarding competition effects 
(cf.~\cref{sec:simulation:results:nonlinearity}).
Moreover, we have also clarified
that not all parts of our analysis in
\cref{sec:theo} require the (common) assumption
of disjoint paths, and why the assumption
is reasonable in the remaining parts.

We are also grateful for the suggestion
to consider dynamic attributes, i.e.,
attributes that are not only set by
an ISP for a certain cost, but also
depend on the demand experienced by the ISP.
For example, the internal-bandwidth attribute
in~\cref{sec:example} might decrease 
if an ISP captures a high demand volume,
similarly as in the selfish-routing literature~\cite{roughgarden2002bad}.
Since such an additional dependency
introduces considerable complexity into the model,
we plan to address this interesting case 
in future work.

\paragraph{Extension of simulation results}
Finally, we have extended our simulation results
and their discussion. In particular,
we now present all our evaluation metrics
segmented by ISP tier, i.e., by `centrality' as
suggested by a reviewer,
and discuss the differences in competition effects
between tiers.
Moreover, we evaluate additional, non-affine 
formulations for valuation and cost
functions in our simulation.
As minor additions, we have also added
details on the maximum path length in
the simulations, on attribute values
reduced by competition, and on total-demand
elasticity.
